Towards Contrastive Learning in Music Video Domain

Contrastive learning is a powerful way of learning multimodal representations across various domains such as image-caption retrieval and audio-visual representation learning. In this work, we investigate if these findings generalize to the domain of music videos. Specifically, we create a dual en-coder for the audio and video modalities and train it using a bidirectional contrastive loss. For the experiments, we use an industry dataset containing 550 000 music videos as well as the public Million Song Dataset, and evaluate the quality of learned representations on the downstream tasks of music tagging and genre classification. Our results indicate that pre-trained networks without contrastive fine-tuning outperform our contrastive learning approach when evaluated on both tasks. To gain a better understanding of the reasons contrastive learning was not successful for music videos, we perform a qualitative analysis of the learned representations, revealing why contrastive learning might have difficulties uniting embeddings from two modalities. Based on these findings, we outline possible directions for future work. To facilitate the reproducibility of our results, we share our code and the pre-trained model.

==> sections/eda.tex <==
%% !TEX root = ../main.tex

\section{Exploratory Data Analysis}

There are 97,241 videos published to the XITE app. We decided to exclude any videos in the category 'other/non-music video' as some videos in this category are not actually music videos. This leaves us with 94,656 music videos that are suitable for our study. Most of these music videos are relatively recent, with 68 percent of the music videos being released in the past ten years. Figure (TODO) presents the complete distribution of release dates in the dataset. Video duration is seemingly normally distributed with a mean of three minutes and 38 seconds, and a standard deviation of 65 seconds. Slightly over half of the music videos originate from either the United States or Great Britain, with the the other half coming from a wide range of other countries (TODO ref figure). The dataset contains music videos from a broad selection of genres. The most prevalent genres in the dataset are pop, regional pop, hip-hop, alternative/indie and latin, which seems to correspond roughly to the general popularity of music genres in western countries, which is the market that XITE is is currently operating in. 

In addition to inspecting different attributes of the metadata, we also explored the audio and video data though the musicnn and 3D Resnet models. Specifically, we sampled 3000 random music videos to explore, and fed them into the networks. For audio, we used only the first X layers(TODO) of the musicnn network, omitting the two dense classification layers. The input was a randomly sampled segment from the audio track and the output was a vector of size 1506. To sample segments from the audio, we split the track into three equally long subsections, and sampled a random segment from each section. To attempt to understand the high dimensional representation of the audio segments better, we used T-SNE dimensionality reduction and plotted the first two components (TODO fig ref). Based on the two dimensional plot of T-SNE scores, there was no clear grouping of the different audio segments. Also, there was no clear relationship between the two first T-SNE scores and metadata features. such as genre or release date. To investigate the feature representations further, we looked at the cosine similarities between feature representations of different audio segments. Fig (TODO) shows that the average cosine similarity between different segments of the same song is higher than the average cosine similarity between segments of different songs. We also explored whether the feature representations of songs of the same genre are more similar than representations for songs of different genres. To do this, we took the same audio segments as before, and calculated a song representation by averaging the feature representations of the different segment of the song. as can be seen in fig (TODO) feature representations for songs of the same genre are not more similar on average than feature representations of songs of two different genres. This corresponds to the T-SNE decomposition, which did not show a clear relationship between feature representations and genre. 

For video, we sampled random segments of video from the same 3000 music videos, and fed them into the 3D Resnet model. As for the audio model, we only used the convolutional layers of the model, meaning that we omitted the final classification layer.

==> sections/research_question.tex <==
% !TEX root = ../main.tex

\section{Task Definition}
\label{sec:task_definition}

==> sections/task_definition.tex <==
% !TEX root = ../main.tex

\section{Task Definition}
\label{sec:task_definition}


==> tables/AUC_per_tag.tex <==
\begin{table}[h]
\caption{Area under the curve per tag for the downstream task of music tagging.}
\label{tauc_per_tag}
\begin{tabular}{lllllllllll}
Type of embeddings          & Country  & Alt Rock & Dance & RnB & indie & \begin{tabular}{@{}c@{}}Female \\ vocals\end{tabular} & Alternative & 80s & Pop& Rock \\
\\ \hline
(B1) Musicnn                & *.8371* & .7845   & .*8476*& *.8837* & *.6980* & .7317    & .7423 & .7861     & .6494 & .8026 \\
(B2) R(2+1)D                & .6293   & .7299   & .7156  & .7527 & .5687     &  .6754   & .5811 & .7299     & .5983 & .6745 \\
(B3) Concatenated           & .8305   & *.7915* & .8431  & .8934 & .6858     & *.7526*  & *.7566* & *.8142* &*.6626*& *.8090* \\
(M1) Contr. audio           & .6325   & .7719   & .7696  & .8468 & .6551    & .5743     & .7364 & .6037     & .6462 & .7827 \\
(M2) Contr. video           & .5371   & .6170   & .6264  & .6842 & .5308    & .6520     & .5781 & .5928     & .5955 & .6789 \\
(M2) Contr. aggregated      & .6180   & .7718   & .7595  & .8424 & .6448    & .6009     & .7311 & .6931     & .6340 & .7860 \\
\hline
\end{tabular}
\end{table}


==> tables/genre_results.tex <==
\begin{table}[h]
\caption{Macro average AUC and $F_1$ \\ score for the downstream task of \\ genre classification.}
\label{genre_results}
\begin{tabular}{lll}
Type of embeddings          & AUC & $F_1$
\\ \hline
(B1) Musicnn                & 0.7902 & 0.1781 \\
(B2) R(2+1)D                & 0.6789 & 0.0531 \\
(B3) Concatenated           & 0.8199 & 0.2060 \\
(M1) Contrastive audio      & 0.6919 & 0.0754 \\
(M2) Contrastive video      & 0.6293 & 0.0437 \\
(M2) Contrastive aggregated &0.6804  & 0.0680 \\
\hline
\end{tabular}
\end{table}
%Macro average AUC and $F_1$ score for the downstream task of genre classification.

==> tables/tagging_results.tex <==
\begin{table}[h]
\caption{Macro average AUC and $F_1$ \\ score for the downstream task of \\ music tagging.}
\label{tag_results}
\begin{tabular}{lll}
Type of embeddings & AUC & $F_1$
\\ \hline
(B1) Musicnn                & 0.7762 & 0.2182 \\
(B2) R(2+1)D                & 0.6566 & 0.0881 \\
(B3) Concatenated           & 0.7839 & 0.2390 \\
(M1) Contrastive audio      & 0.7019 & 0.1040 \\
(M2) Contrastive video      & 0.6092 & 0.0934 \\
(M2) Contrastive aggregated & 0.7082 & 0.1051 \\
\hline
\end{tabular}
\end{table}

% Macro average AUC and $F_1$ score for the downstream task of music tagging.
